On the Relationship Between the Developer's Perceptible Race and Ethnicity and the Evaluation of Contributions in OSS

Open Source Software (OSS) projects are typically the result of collective efforts performed by developers with different backgrounds. Although the quality of developers' contributions should be the only factor influencing the evaluation of the contributions to OSS projects, recent studies have shown that diversity issues are correlated with the acceptance or rejection of developers' contributions. This paper assists this emerging state-of-the-art body on diversity research with the first empirical study that analyzes how developers' perceptible race and ethnicity relates to the evaluation of the contributions in OSS. We performed a large-scale quantitative study of OSS projects in GitHub. We extracted the developers' perceptible race and ethnicity from their names in GitHub using the Name-Prism tool and applied regression modeling of contributions (i.e, pull requests) data from GHTorrent and GitHub. We observed that among the developers whose perceptible race and ethnicity was captured by the tool, only 16.56% were perceptible as Non-White developers; contributions from perceptible White developers have about 6-10% higher odds of being accepted when compared to contributions from perceptible Non-White developers; and submitters with perceptible non-white races and ethnicities are more likely to get their pull requests accepted when the integrator is estimated to be from their same race and ethnicity rather than when the integrator is estimated to be White. Our initial analysis shows a low number of Non-White developers participating in OSS. Furthermore, the results from our regression analysis lead us to believe that there may exist differences between the evaluation of the contributions from different perceptible races and ethnicities. Thus, our findings reinforce the need for further studies on racial and ethnic diversity in software engineering to foster healthier OSS communities.

==> description.tex <==

Since there is little empirical evidence of perceptible racial and ethnic diversity based involvement in GitHub, we gathered the demographics of GitHub developers. This allow us to make inferences about the perceptible race and ethnicity in the GitHub's community, and to quantitatively demonstrate the presence or lack of diversity in the community. This section describes the demographics (i.e, race and ethnicity, and geographical location) of the developers who participated in the $2,507,591$ pull requests that survived the filtering explained in \ref{sec:pr_selection}. 

%There is little empirical evidence of perceptible racial and ethnic diversity based involvement in GitHub. Thus, we gathered the demographics of GitHub developers to make inferences about the perceptible race and ethnicity in the community, and to quantitatively demonstrate the presence or lack of diversity in GitHub's community. %From the $2,507,591$ pull requests that survived the filtering explained in \ref{sec:pr_selection}, we extracted the pull request acceptance status, the developers' perceptible race and ethnicity, and the developers' geographical location.

%From the $2,507,591$ pull requests, we extracted the pull request acceptance status, the developers' perceptible race and ethnicity, and the developers' geographical location. While the distribution of developers with publicly recognizable perceptible race and ethnicity in GitHub is  57.2\%, 42.8\% of GitHub developers were classified as ``Unknown''.

\begin{table*}
\centering
\renewcommand{\arraystretch}{1.2}
\caption{Races and Ethnicities population description}
\label{tab:eth_dist}
\begin{tabular}{l|cl|cl|cl}
\toprule
         & \multicolumn{2}{c|}{Number of Developers} & \multicolumn{2}{c|}{Number of pull requests submitted by} & \multicolumn{2}{c}{Number of pull requests integrated by} \\ 
         & Population        & Proportion(\%)       & Population               & Proportion(\%)              & Population                 & Proportion(\%)                \\ \cline{2-7} 
White    & 235541            & 47.8   \%              & 1543967                  & 61.57 \%                  & 1762204                    & 70.28   \%                      \\
API      & 33776             & 6.8   \%               & 162792                   & 6.49     \%                   & 122656                     & 4.89     \%                     \\
Hispanic & 12356             & 2.5    \%              & 64567                    & 2.57     \%                   & 74583                      & 2.97      \%                    \\
Black    & 638               & 0.1    \%              & 3092                     & 0.13      \%                  & 2090                       & 0.08      \%                    \\
AIAN     & 1                 & $\approx 0$    \%      & 3                        & $\approx 0$   \%              & 0                          & 0           \%                  \\
Unknown  & 210858            & 42.8      \%           & 733170                   & 29.24       \%                & 546058                     & 21.78      \%                   \\ \hline
Total    & 493170            & 100     \%             & 2507591                  & 100         \%                & 2507591                    & 100\% \\\hline \bottomrule                        
\end{tabular}
\end{table*}

\subsection{Perceptible racial and ethnic distribution in GitHub}
From the $493,170$ developers in our dataset, while we classified the perceptible race and ethnicity of $282,312$ developers (57.2\%), $210,858$ (42.8\%) developers were classified as ``Unknown''. Furthermore, 96\% of the $250,759$ pull requests in our dataset were submitted by contributors outside the projects. Table~\ref{tab:eth_dist} shows a low number of perceptible Non-White developers in GitHub (6.8\% perceptible API developers, 2.5\% perceptible Hispanic developers, 0.1\% perceptible Black developers, and $\approx 0\%$ perceptible AIAN developers) when compared to the number of perceptible White developers (47.8\%). Table~\ref{tab:eth_dist} also indicates that (1) perceptible White developers submit six times more (61.57\%) pull requests than perceptible Non-White developers ($6.49 + 2.57 + 0.13 = 9.19$), and (2) perceptible White developers integrate ten times more (70.28\%) pull requests than perceptible Non-White developers ($4.89 + 2.97 + 0.08 = 7.94$). %While the above two findings already indicate a serious diversity issue with OSS communities in GitHub, the fact that there is a higher percentage of perceptible White integrators than submitters indicates that when it comes to positions of power (integrator) in an OSS environment there is an even higher lack of diversity. We will discuss more about this is Section~\ref{sec:disc}.

Table \ref{tab:eth_dist} also shows the percentage number of pull request contributions submitted and integrated by each perceptible race and ethnicity. While the vast majority of contributions (61.57\%) were submitted by developers perceptible as White, developers perceptible as API, Hispanic, Black, and AIAN, in total, have submitted less than 10\% of the contributions. 29.24\% of contributions were submitted by developers with ``Unknown'' perceptible race and ethnicity.

\subsection{Acceptance rate of each perceptible race and ethnicity in GitHub }
Table~\ref{fig:general_acc} shows the general acceptance rate for each group. While the highest acceptance rate among all perceptible races and ethnicities is that of perceptible White submitter with 82.6\%, the acceptance rate average of perceptible API, Hispanic, and Black submitters is 80.04\%, 81.59\%, and 81.34\%, respectively. An interesting result shows that the lowest acceptance rate is that of ``Unknown'' perceptible race and ethnicity with 79.2\%. 

%\begin{figure}
%\centering
%  \includegraphics[width=\linewidth]{img/acceptance_general_bw.png}
%\caption{Pull Request acceptance rate (represented in percentage) per racial and ethnic group}
%\label{fig:general_acc} 
%\end{figure}

\begin{table}
\centering
  \caption{Pull Request acceptance rate (represented in percent-age) per racial and ethnic group.}
  \label{fig:general_acc}
  \begin{tabular}{llllll}
    \toprule
    Status PR & Unknown & White & API & Hispanic & Black\\
    \midrule
    Rejected  & 20.8 & 17.4 & 19.96 & 18.41 & 18.66\\
    Accepted & 79.2 & 82.6 & 80.04 & 81.59 & 81.34\\ \hline
  \bottomrule
\end{tabular}
\end{table}

We also analyzed the distribution of developers and pull request acceptance rates between different groups when considering the integrator's perceptible race and ethnicity. For that, we calculated the acceptance rate of each developer against each integrator. We found that perceptible White submitters have an acceptance rate average of (73\%) when the integrator is also perceptible as White (but their acceptance rate average is (69\%) when measured against all integrators). The acceptance rate average of submitter-integrator pairs perceptible as API and Hispanic (when the submitter and integrator are perceptible to be in the same group) is 78\% and 76\%, respectively. In addition, we found that this average is higher than the cases where the integrator is perceptible as a White developer. This average is 69\% for perceptible API-White developer pairs and 71\% for perceptible Hispanic-White developer pairs. These differences are worthy of investigation because a preliminary analysis showed statistically significant differences between the pull request acceptance rate of each perceptible racial and ethnic group. We have added more details about the preliminary analysis in Sections 4.1 and 4.2 in our online appendix (B)~\cite{repro}.


\subsection{Country distribution of each perceptible racial and ethnic group in GitHub}

Among $493,170$ developers, we identified the country of $245,881$ (49.85\%) of them. Figure~\ref{fig:top10} shows the top countries identified based on the number of developers. North American countries: U.S. and Canada, count for 17.24\% of developers. The top European countries: Germany, UK, France, and the Netherlands, count for 13.03\% of developers. Russia, China, and India also appear in the top countries, with 5.18\% of developers. 


\begin{figure}[t]
\centering
  \includegraphics[width=\linewidth]{img/top10.png}
\caption{Top Countries according to the number of developers}
\label{fig:top10} 
\end{figure}


We looked at the top five countries for each racial and ethnic group based on the number of developers as a soundness check for the perceptible race and ethnicity classification method. This process resulted in only fourteen distinct countries since three countries (U.S., UK, Canada) were among the top countries for different races and ethnicities. For U.S., $87.09\%$ were perceptible as White users, $10.13\%$ were perceptible as API users, $2.59\%$ were perceptible as Hispanic users, and only $0.17\%$ were perceptible as Black users. For UK, $93.56\%$ were perceptible as White users, $3.71\%$ were perceptible as API users, $2.52\%$ were perceptible as Hispanic users, and only $0.19\%$ were perceptible as Black users. In Canada, $88.23\%$ were perceptible as White users, $9.56\%$ were perceptible as API users, $1.88\%$ were perceptible as Hispanic users, and only $0.31\%$ were perceptible as Black users. Each cell in Figure~\ref{fig:heatmap} shows what proportion of the race and ethnicity resides in each country. The percentage numbers in Figure~\ref{fig:heatmap} are normalized using the IPFP (Iterative Proportional Fitting Procedure) function~\cite{fienberg1981iterative} of the TeachingSampling~\footnote{\url{https://rdrr.io/cran/TeachingSampling/man/IPFP.html}} package in R. From Figure~\ref{fig:heatmap}, we can observe that (1) the U.S. has the highest percentage of the perceptible Hispanic developers, perceptible API developers, perceptible White developers, and perceptible Black developers (the highest percentage in the U.S. is perceptible White developers); (2) besides the U.S., most of the perceptible API developers reside in Asian countries; (3) European and North American countries represent a higher proportion of perceptible White developers; (4) besides the U.S., South American countries and Spain represent a higher proportion of perceptible Hispanic developers; and (5) other than U.S., African countries have a higher proportion of perceptible Black developers.

%We can observe that inferring race and ethnicity from countries may not be accurate because each country can have more than one racial and ethnic group. 
Figure \ref{fig:heatmap} shows that although the largest perceptible racial and ethnic group of developers in France and Germany is White, there are developers from these countries who are perceptible as Black developers and as Hispanic developers. Furthermore, for perceptible White countries such as Canada or U.S. the percentage of perceptible API developers is also considerable. %These results indicate which countries participating in GitHub are ethnically more diverse.

\begin{figure}[b]
  \includegraphics[width=\linewidth]{img/heatmap.png}
\caption{perceptible race and ethnicity population proportion in the top countries}
\label{fig:heatmap} 
\end{figure}

